RuAG: Learned-rule-augmented Generation for Large Language Models

In-context learning (ICL) and Retrieval-Augmented Generation (RAG) have gained attention for their ability to enhance LLMs' reasoning by incorporating external knowledge but suffer from limited contextual window size, leading to insufficient information injection. To this end, we propose a novel framework, RuAG, to automatically distill large volumes of offline data into interpretable first-order logic rules, which are injected into LLMs to boost their reasoning capabilities. Our method begins by formulating the search process relying on LLMs' commonsense, where LLMs automatically define head and body predicates. Then, RuAG applies Monte Carlo Tree Search (MCTS) to address the combinational searching space and efficiently discover logic rules from data. The resulting logic rules are translated into natural language, allowing targeted knowledge injection and seamless integration into LLM prompts for LLM's downstream task reasoning. We evaluate our framework on public and private industrial tasks, including natural language processing, time-series, decision-making, and industrial tasks, demonstrating its effectiveness in enhancing LLM's capability over diverse tasks.

==> AandB_code.tex <==
\begin{lstlisting}[language=Python, style=codestyle, caption=Alice\&Bob Python Code Snippets, label=lst:AandB]
import numpy as np
import matplotlib.pyplot as plt
from matplotlib.gridspec import GridSpec
import cv2

class Alice_and_Bob(object):
    def __init__(self, map_size=(13, 9), n=2):
        self.length, self.width = map_size
        self.agent_num = n
        self.generate_map()
        self.map_ = {'agent':{0: 5, 1: 6}, 'key':{0: 2, 1: 3}, 'lever': 4, 'treasure': 7, 'wall': 1}

    def generate_map(self):
        self.occupancy = np.zeros((self.length, self.width))
        
        # initialize agents
        self.agt_pos = [[1, 1], [1, self.width-2]]
        self.occupancy[self.agt_pos[0][0]][self.agt_pos[0][1]] = 5
        self.occupancy[self.agt_pos[1][0]][self.agt_pos[1][1]] = 6

        # enclose the surroundings
        for i in range(self.length):
            self.occupancy[i, 0] = 1
            self.occupancy[i, self.width - 1] = 1
        for i in range(self.width):
            self.occupancy[0, i] = 1
            self.occupancy[self.length -1, i] = 1
        
        # build walls
        for i in range(1,9):
            self.occupancy[i, 4] = 1
        for i in range(1,5):
            self.occupancy[8, i] = 1
        for i in range(5,8):
            self.occupancy[4, i] = 1
        self.occupancy[10, 6] = 1
        self.occupancy[10, 7] = 1
        self.occupancy[11, 6] = 1
        self.secret_wall_pos = [[10, 6], [10, 7], [11, 6]]

        # generate keys and doors
        self.keys_pos = [[3, 5], [11, 1]]
        self.doors_pos = [[8, 2], [4, 6]]
        self.lever_pos = [5, 7]
        self.occupancy[self.keys_pos[0][0]][self.keys_pos[0][1]] = 2
        self.occupancy[self.keys_pos[1][0]][self.keys_pos[1][1]] = 3
        self.occupancy[self.lever_pos[0]][self.lever_pos[1]] = 4
        self.lever_in_use = False

        # initialize treasure
        self.treasure_pos = [11, 7]
        self.occupancy[self.treasure_pos[0]][self.treasure_pos[1]] = 7
        
    def reset(self):
        self.generate_map()
        obs = self.get_obs()
        return obs

    def step(self, action_list):
        reward = 0
        info = [0, 0]
        # agent move
        for i in range(self.agent_num):
            if action_list[i] == 0:  # move up
                if self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]+1] != 1:
                    self.agt_pos[i][1] = self.agt_pos[i][1] + 1
                    self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]-1] = 0
                    self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]] = 5+i
                else:
                    reward = reward - 0.1
            elif action_list[i] == 1:  # move down
                if self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]-1] != 1:
                    self.agt_pos[i][1] = self.agt_pos[i][1] - 1
                    self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]+1] = 0
                    self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]] = 5+i
                else:
                    reward = reward - 0.1
            elif action_list[i] == 2:  # move left
                if self.occupancy[self.agt_pos[i][0]-1][self.agt_pos[i][1]] != 1:
                    self.agt_pos[i][0] = self.agt_pos[i][0] - 1
                    self.occupancy[self.agt_pos[i][0]+1][self.agt_pos[i][1]] = 0
                    self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]] = 5+i
                else:
                    reward = reward - 0.1
            elif action_list[i] == 3:  # move right
                if self.occupancy[self.agt_pos[i][0]+1][self.agt_pos[i][1]] != 1:
                    self.agt_pos[i][0] = self.agt_pos[i][0] + 1
                    self.occupancy[self.agt_pos[i][0]-1][self.agt_pos[i][1]] = 0
                    self.occupancy[self.agt_pos[i][0]][self.agt_pos[i][1]] = 5+i
                else:
                    reward = reward - 0.1

        # check keys
        for i in range(self.agent_num):
            for j in range(len(self.keys_pos)):
                if self.agt_pos[i] == self.keys_pos[j]:
                    self.occupancy[self.doors_pos[j][0]][self.doors_pos[j][1]] = 0
                    info[i] = self.map_['key'][j]
        
        # check lever
        if (self.agt_pos[0] == self.lever_pos or self.agt_pos[1] == self.lever_pos) and not self.lever_in_use:
            self.occupancy[10][6] = 0  # clear the wall
            self.occupancy[10][7] = 0  # clear the wall
            self.occupancy[11][6] = 0  # clear the wall
            self.lever_in_use = True
            if self.agt_pos[0] == self.lever_pos:
                info[0] = self.map_['lever']
            else: info[1] = self.map_['lever']
                
        elif not (self.agt_pos[0] == self.lever_pos or self.agt_pos[1] == self.lever_pos):
            if self.agt_pos[0] not in self.secret_wall_pos and self.agt_pos[1] not in self.secret_wall_pos:
                self.occupancy[10][6] = 1  # reset the wall
                self.occupancy[10][7] = 1  # reset the wall
                self.occupancy[11][6] = 1  # reset the wall
                self.occupancy[self.lever_pos[0]][self.lever_pos[1]] = 4
                self.lever_in_use = False
            elif self.agt_pos[0] in self.secret_wall_pos:
                self.agt_pos[0] = [9, 5] # bounce back to specific pos
                self.occupancy[self.agt_pos[0][0]][self.agt_pos[0][1]] = 5

                self.occupancy[10][6] = 1  # reset the wall
                self.occupancy[10][7] = 1  # reset the wall
                self.occupancy[11][6] = 1  # reset the wall
                self.occupancy[self.lever_pos[0]][self.lever_pos[1]] = 4
                self.lever_in_use = False
                reward -= 10
            elif self.agt_pos[1] in self.secret_wall_pos:
                self.agt_pos[1] = [9, 5] # bounce back to specific pos
                self.occupancy[self.agt_pos[1][0]][self.agt_pos[1][1]] = 6

                self.occupancy[10][6] = 1  # reset the wall
                self.occupancy[10][7] = 1  # reset the wall
                self.occupancy[11][6] = 1  # reset the wall
                self.occupancy[self.lever_pos[0]][self.lever_pos[1]] = 4
                self.lever_in_use = False
                reward -= 10
        
        done = False
        
        # check treasure
        if self.agt_pos[0] == self.treasure_pos or self.agt_pos[1] == self.treasure_pos:
            reward = reward + 100
            if self.agt_pos[0] == self.treasure_pos:
                info[0] = self.map_['treasure']
            else: info[1] = self.map_['treasure']
            done = True
        
        next_obs = self.get_obs()
        return next_obs, reward, done, info

    def get_partial_obs(self, i):
        partial_obs = self.occupancy[self.agt_pos[i][0]-1:self.agt_pos[i][0]+2,self.agt_pos[i][1]-1:self.agt_pos[i][1]+2].reshape(1,-1)
        rel_dis_teammate = np.array(self.agt_pos[1-i]) - np.array(self.treasure_pos)
        rel_dis = np.array(self.agt_pos[i]) - np.array(self.treasure_pos)
        return np.concatenate([np.squeeze(partial_obs), rel_dis_teammate, rel_dis])
        # return np.concatenate([np.squeeze(partial_obs), self.agt_pos[1-i], rel_dis])

    def get_obs(self):
        return [self.get_partial_obs(i) for i in range(self.agent_num)]
\end{lstlisting}
